Massive Star-Forming Galaxies Have Converted Most of Their Halo Gas into Stars

In the local Universe, the efficiency for converting baryonic gas into stars is very low. In dark matter halos where galaxies form and evolve, the average efficiency varies with galaxy stellar mass and has a maximum of about twenty percent for Milky-Way-like galaxies. The low efficiency at higher mass is believed to be produced by some quenching processes, such as the feedback from active galactic nuclei. We perform an analysis of weak lensing and satellite kinematics for SDSS central galaxies. Our results reveal that the efficiency is much higher, more than sixty percent, for a large population of massive star-forming galaxies around $10^{11}M_{\odot}$. This suggests that these galaxies acquired most of the gas in their halos and converted it into stars without being affected significantly by quenching processes. This population of galaxies is not reproduced in current galaxy formation models, indicating that our understanding of galaxy formation is incomplete. The implications of our results on circumgalactic media, star formation quenching and disc galaxy rotation curves are discussed. We also examine systematic uncertainties in halo-mass and stellar-mass measurements that might influence our results.

==> old.tex <==
\usepackage[utf8]{inputenc}

\title{High Conversion Efficiency for Massive Star-Forming Galaxies}
\author{Huiyuan Wang}
\date{November 2021}

\begin{document}

\maketitle

\section{Introduction}

\end{document}

